Machine learning quantum data to accelerate quantum Monte Carlo

Simulating strongly correlated electrons in molecules and materials remains a central goal for quantum computing. A promising strategy uses quantum processors to prepare trial wavefunctions that guide classical quantum Monte Carlo (QMC). However, the enormous computational cost of repeatedly processing quantum measurements has severely limited the practical scalability of this approach. Here, we overcome this bottleneck by compressing quantum measurement data into machine-learning models that efficiently provide the wavefunction overlaps needed by QMC. This accelerates quantum-classical QMC by orders of magnitude, enabling chemically accurate simulations on up to 40 qubits, more than doubling the scale of previous hardware demonstrations with comparable accuracy. We demonstrate our approach on hydrogen chains and strongly correlated iron-sulfur clusters using measurements from Google's Willow processor. By enabling efficient reuse of quantum-state information on the classical coprocessor, our framework addresses a fundamental bottleneck in hybrid quantum algorithms that will persist even into the fault-tolerant era.

==> splitrefs.tex <==
% Split references in a REVTeX 4.2 manuscript using apsrev4-2.bst.
\makeatletter

% Record every key cited before the main bibliography, including in captions.
\let\SR@addkey\NAT@cite@list@append
\def\NAT@cite@list@append#1{%
  \SR@addkey{#1}%
  \expandafter\gdef\csname SR@main@\@citeb\endcsname{}}

% APS ends each generated entry with \BibitemShut{...}.
\long\def\SR@skip#1\BibitemShut#2{}
\newcommand{\SR@filter}[2]{%
  \let\SR@ifmain#1\let\SR@ifsi#2%
  \def\bibitem[##1]##2{%
    \ifcsname SR@main@##2\endcsname
      \expandafter\SR@ifmain
    \else
      \expandafter\SR@ifsi
    \fi[##1]{##2}}}

\newcommand{\MainReferences}[1]{%
  \let\NAT@cite@list@append\SR@addkey
  \auto@bib@empty
  \let\SR@bibitem\bibitem
  \begingroup
    \SR@filter\SR@bibitem\SR@skip
    \bibliography{#1}%
    \xdef\SR@last{\arabic{NAT@ctr}}%
  \endgroup}

\newcommand{\SupplementaryReferences}{%
  \begingroup
    \def\bibsection{\section*{Supplementary References}}%
    \def\thebibliography##1{%
      \NAT@thebibliography{##1}\setcounter{NAT@ctr}{\SR@last}}%
    \let\endthebibliography\endNAT@thebibliography
    \SR@filter\SR@skip\SR@bibitem
    \InputIfFileExists{\jobname.bbl}{}{}%
  \endgroup}
\makeatother

